A Comparison of Semi-Supervised Learning Techniques for Streaming ASR at Scale

Unpaired text and audio injection have emerged as dominant methods for improving ASR performance in the absence of a large labeled corpus. However, little guidance exists on deploying these methods to improve production ASR systems that are trained on very large supervised corpora and with realistic requirements like a constrained model size and CPU budget, streaming capability, and a rich lattice for rescoring and for downstream NLU tasks. In this work, we compare three state-of-the-art semi-supervised methods encompassing both unpaired text and audio as well as several of their combinations in a controlled setting using joint training. We find that in our setting these methods offer many improvements beyond raw WER, including substantial gains in tail-word WER, decoder computation during inference, and lattice density.

==> figures/DecodingTable.tex <==
\begin{table*}[t]
\begin{minipage}{.5\linewidth}
\centering
\begin{tabular}{||c|c|c|c|c|c||} 
 \hline
 Model & \textbf{VS} & \textbf{Noisy} & \textbf{RPN} & \textbf{R\_LM} & \textbf{C\_LM} \\ [0.5ex] 
 \hline\hline
 \textbf{E-0} & 162 & 187 & 297 & 357 & 325 \\ 
 \hline
 \textbf{E-A} & 151 & 177 & 264 & 321 & 296 \\ 
 \hline
 \textbf{E-B} & 151 & 177 & 268 & 327 & 301\\ 
 \hline
 \textbf{E-C} & 147 & 174 & 277 & 336 & 209\\ 
 \hline
 \textbf{E-AB} & 151 & 178 & 279 & 339 & 312\\
 \hline
 \textbf{E-AC} & 147 & 175 & 265 & 324 & 298\\ 
 \hline
 \textbf{E-ABC} & 149 & 176 & 268 & 326 & 300\\ 
 \hline
\end{tabular}
\centering
\caption{Average Decoding States}
\label{table:average_decoding_states}
\end{minipage}
\begin{minipage}{.5\linewidth}
\centering
\begin{tabular}{||c|c|c|c|c|c||} 
 \hline
 Model & \textbf{VS} & \textbf{Noisy} & \textbf{RPN} & \textbf{R\_LM} & \textbf{C\_LM}  \\ [0.5ex] 
 \hline\hline
 \textbf{E-0} & 3.2 & 3.3 & 6.2 & 8.1 & 9.7\\ 
 \hline
 \textbf{E-A} & 3.6 & 3.8 & 6.4 & 8.4 & 10.0\\ 
 \hline
 \textbf{E-B} & 3.6 & 3.7 & 6.4 & 8.4 & 10.0\\ 
 \hline
 \textbf{E-C} & 3.6 & 3.7 & 6.4 & 8.4 & 10.0\\ 
 \hline
 \textbf{E-AB} & 3.6 & 3.7 & 6.3 & 8.4 & 10.0\\ 
 \hline
 \textbf{E-AC} & 3.6 & 3.7 & 6.4 & 8.5 & 10.1 \\ 
 \hline
 \textbf{E-ABC} & 3.6 & 3.7 & 6.4 & 8.5 & 10.0\\ 
 \hline
\end{tabular}
\centering
\caption{Lattice Density}
\label{table:lattice_density}
\end{minipage}
\end{table*}


==> figures/WERTable.tex <==
\begin{table}[h]
\centering
\begin{tabular}{||c|c|c|c|c|c||} 
 \hline
 Model & \textbf{VS} & \textbf{Noisy} & \textbf{RPN} & \textbf{R\_LM} & \textbf{C\_LM} \\ [0.5ex] 
 \hline\hline
 \textbf{E-0} & 6.0 & 8.2 & 21.2 & 38.3 & 55.8 \\ 
 \hline
 \textbf{E-A} & 6.0 & 8.3 & 20.1 & 36.4 & 54.5 \\ 
 \hline
 \textbf{E-B} & 6.0 & 8.1 & 21.0 & 37.5 & 55.4 \\ 
 \hline
 \textbf{E-C} & 6.0 & 8.3 & 21.3 & 38.3 & 55.6 \\ 
 \hline
 \textbf{E-AB} & 6.0 & 8.3 & 20.3 & 36.7 & 54.7 \\ 
 \hline
 \textbf{E-AC} & 6.0 & 8.2 & 20.5 & 37.2 & 55.1 \\ 
 \hline
 \textbf{E-ABC} & 6.0 & 8.4 & 20.4 & 36.9 & 55.0\\ 
 \hline
\end{tabular}
\centering
\caption{Word Error Rate}
\label{table:wer_table}
\end{table}


==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Methods for learning from large-scale supervised datasets were the primary driver of progress in speech processing from the HMM/GMM era \cite{FourResearchGroups} well into the era of deep learning \cite{RNNT, LAS, ASSAP_ASR}.  However, as the scope of ASR research has expanded into challenging settings such as low-resource languages and difficult acoustic conditions, it has become difficult to gather large-scale in-domain supervised datasets \cite{2013LowResource}.  In recent years, much of the speech community's attention has moved to alternatives to purely supervised learning.

Semi-supervised \cite{LitReviewDeepSemisupLearning} learning has emerged as a powerful paradigm for addressing contemporary problems in speech recognition \cite{LitReviewSemisupSpeech_Thesis}.  In a semi-supervised training scheme, unpaired speech and/or text examples supplement a supervised dataset to provide greater acoustic/language coverage.  A broad literature has emerged exploring various mechanisms for incorporating speech-only \cite{Wav2Vec, APC, WavLM} and text-only \cite{ShallowFusion, ColdFusion, FusionComparison} data into ASR training.  

Many of the strongest methods in semi-supervised speech processing can be seen as chasing the success of Masked Language Modeling (MLM) in natural language processing, as exemplified by BERT \cite{BERT}. On the whole, MLM-based methods have demonstrated a substantial improvement in ASR performance \cite{Wav2Vec2_0, HuBERT, WavLM}.  The WER improvements are demonstrated specifically in large-parameter, full-context models, and are especially strong when only a small amount of supervised data is available.  However, WER improvements are generally minimal when supplementing an already-large supervised dataset (for example, see 960hr Librispeech results in \cite{Wav2Vec2_0}), and are relatively unreported on for on-device-sized, streaming architectures.

In this work, we study MLM for ASR in both the speech and text domains in the context of a very large supervised dataset ($\approx$ 200k hours).  We compare these methods to TTS pesudolabeling, a more conventional method of semisupervised learning.  We specifically study a streaming model that is sufficiently small to run on-device ($\approx$ 164M parameters), and present results targeting realistic production considerations.  Our main contributions are as follows:

\begin{enumerate}
    \item We present an architecture capable of any combination MLM for unpaired text, MLM for unpaired audio, and TTS pseudolabeling.  We provide insights on how to train such a model.
    \item We compare methods and combinations of methods not only by raw WER, but also by performance on a variety of challenging acoustic and language conditions.  We demonstrate that even in the presence of a very large supervised dataset, unlabeled data yields improvements. 
    \item We present a novel study of quantities other than WER that are relevant to production, on-device deployment.  In particular, we take measurements of the richness of the lattice (which is useful to downstream NLU tasks) and the CPU cost of decoding.  We demonstrate that unlabeled data yields surprising improvements on these important metrics.  
\end{enumerate}

The rest of this work is structured as follows.  Section \ref{sec:methods} gives our architecture and mechanisms for consuming unpaired data.  Section \ref{sec:experiments} details our experiments and evaluation criterion.  Section \ref{sec:results} presents results and analysis, and Section \ref{sec:conclusions} concludes.
